What Drives Liquidity on Decentralized Exchanges? Evidence from the Uniswap Protocol

We study liquidity on decentralized exchanges (DEXs), identifying factors at the platform, blockchain, token pair, and liquidity pool levels with predictive power for market depth metrics. We introduce the v2 counterfactual spread metric, a novel criterion which assesses the degree of liquidity concentration in pools using the ``concentrated liquidity'' mechanism, allowing us to decompose the effect of a factor on market depth into two channels: total value locked (TVL) and concentration. We further explore how external liquidity from competing DEXs and private inventory on DEX aggregators influence market depth. We find that (i) gas prices, returns, and a DEX's share of trading volume affect liquidity through concentration, (ii) internalization of order flow by private market makers affects TVL but not the overall market depth, and (iii) volatility, fee revenue, and markout affect liquidity through both channels.

==> sections/5.Extension.tex <==
\section{Extension: External Liquidity}

% \subsection{Impact of External Liquidity on Spread}

The success of AMMs has lead to the proliferation of DEXs, with there being over one hundred DEXs at the time of writing. 
The increase in competition between DEXs introduces challenges such as the fragmentation of liquidity across multiple liquidity pools and DEXs. 
In addition, the introduction of DEX aggregators has led to new methods for order routing, leveraging liquidity from various on-chain sources and off-chain private market makers (PMMs). While these services improve outcomes for swappers \cite{bachu2024quantifying}, PMMs earn fees that would have otherwise gone to on-chain LPs, affecting their overall profitability.
% Recent research (\cite{bachu2024quantifying}) has measured the price improvements offered by order flow aggregators like UniswapX and 1inch, finding average price improvements of 4 to 5 basis points for users.

% Despite the successful innovations brought by \amms, these designs face challenges such as fragmented liquidity across multiple \dexs or liquidity pools. 
% In response to these challenges, leading \dexs like Uniswap, 1inch, and others have introduced new methods for handling orders, leveraging liquidity from various off-chain sources or private liquidity providers to facilitate trades to optimize trading outcomes for participants. 
% Recent research by \cite{bachu2024quantifying} has measured the price improvements offered by Order Flow Aggregators (OFAs) like UniswapX and 1inch and found an average price improvement of 4 to 5 basis points for users.

% Competition between DEXs and the introduction of aggregator services have important implications for on-chain liquidity provision. 
% From one DEX's point of view, competing DEXs take away swap volume, and aggregator services reduce the volume of swaps that directly interact with AMMs by routing swaps away to be filled by private liquidity sources.
% These factors potentially influence spreads, overall liquidity, and the revenue generated by on-chain LPs. 

% This shift in routing raises key questions about the sustainability of on-chain liquidity provision in the presence of competing private liquidity sources.

% The introduction of these liquidity services has important implications for on-chain liquidity provision. 
% By routing trades away from on-chain pools, these services can reduce the volume of swaps that directly interact with AMMs, potentially influencing the bid-ask spread, overall liquidity, and the revenue generated by on-chain liquidity providers. 
% This shift in trade routing raises key questions about the sustainability of on-chain liquidity provision in the presence of competing private liquidity sources.

\subsection{Measuring External Liquidity}

To better understand how these external liquidity sources might affect on-chain liquidity provision, we introduce variables that (i) capture the volume of swaps taking place on other DEXs and (ii) filled by private liquidity due to aggregator routing.
Using data from Dune Analytics, we track swap volume on other DEXs and routed through aggregators, isolating swaps filled completely by private liquidity by comparing transaction hashes with on-chain events. 
A simple heuristic to identify these types of swaps is to take all swaps emitting events to aggregator trackers that did not emit a swap event to on-chain data trackers. 
% From this, we compute the \textit{DEX competitor trading volume share} and \textit{internalization ratio}, defined as follows.

\paragraph{\textbf{Competitor Market Share}.} 
For a set $\mathcal{D}$ of DEXs (including the given DEX) and a chain-pair, we compute the fraction of trading volume for that chain-pair occurring outside of the given DEX on day $t$:\footnote{Typically, market share for DEXs is evaluated in terms of trading volume. As a single DEX can have several pools trading a pair on a chain, we require a platform-level metric to assess competition and trader's sentiments towards a given DEX.}
\begin{align*}
    \textsf{CompetitorShare}_t^{chain,pair} = 1-\frac{v_t}{\sum_{D\in\mathcal{D}}v_t^D}
\end{align*}
where $v_t$ and $v_t^D$ are the swap volumes on the given DEX and DEX $D$ in USD, respectively, for a given chain-pair on day $t$. 

\paragraph{\textbf{Internalization Ratio.}}
Given a set $\mathcal{D}$ of DEXs, a set $\mathcal{A}$ of aggregators, and a chain-pair, we compute the proportion of swap volume routed or internalized by private market makers active on $\mathcal{A}$, henceforth referred to as ``private volume,'' to the total on-chain plus private volume for that chain-pair on day $t$:\footnote{Since an aggregator could route trades to a variety of DEXs, we need $\mathcal{D}$ to include all DEX that the aggregators in $\mathcal{A}$ may route to.}
\begin{align*}
    \textsf{Internalization}_t^{chain,pair} = \frac{\sum_{A\in\mathcal{A}}v_t^A}{\sum_{D\in\mathcal{D}}v_t^D+\sum_{A\in\mathcal{A}}v_t^A}
\end{align*}
where $v_t^A$ is the private volume on aggregator $A$ and $v_t^D$ is the swap volume on DEX $D$, both in USD, for a given chain-pair on day $t$. 

\paragraph{\textbf{Extended Regression Model.}}
We take $\mathcal{D}$ as the 130 DEXs whose swap events are tracked on Dune Analytics and $\mathcal{A}$ as the 13 aggregators whose swap events are tracked on Dune Analytics.
We add the competitor market share and internalization ratio variables to the baseline model and estimate the model with the dependent variable specifications in models (\ref{equation1})--(\ref{equation3}):
% We take $\mathcal{D}$ to be the set of all 130 DEXs whose swap events are tracked on Dune Analytics. 
% Since we only include Uniswap liquidity pools in our sample, the competitor market share is simply the ratio of Uniswap volume to total DEX volume for a given chain-pair in our case. 
% We consider two different aggregator sets $\mathcal{A}$, one that includes all 13 aggregators whose swaps are tracked on Dune Analytics, and another that only contains UniswapX. \footnote{Swaps on UniswapX filled by private liquidity are not tracked on Dune.}
% We add these variables to the baseline model and estimate the model using the dependent variable specifications in models (\ref{equation1})--(\ref{equation3}):
%We then posit the following regression framework adapted from \autoref{equation1}. Further more, similar to the previous section, we also analysis the decomposition like in \autoref{equation2} and \autoref{equation3} with different dependent variable specification.
\begin{align}
y_{t+1}^{pool} &= \beta_0 
                    + \beta_1 \log\textsf{GasPrice}_t^{chain} 
                    + \beta_2\textsf{\,LogReturns}_t^{pair} 
                    + \beta_3{\textsf{\,Volatility}}_t^{pair} \notag \\
                    & + \beta_4 \log\textsf{FeeRevenue}_t^{pool}
                    + \beta_5{\textsf{\,Markout}}_t^{pool} 
                    + \beta_6{\textsf{\,CompetitorShare}}_t^{chain,pair} \notag \\       
                    & + \beta_7{\textsf{\,Internalization}}_t^{chain,pair} 
                    + \gamma^\textit{pool} + \delta_t + \varepsilon_{t+1}^{pool}
\label{equation4}
\end{align}
where $y\in\{\log\textsf{v3Spread},\,\log\textsf{cfv2Spread},\log\textsf{v3S/cfv2S}\}$.\footnote{We performed robustness checks similar to those in footnote 4.}

\subsection{Results and Discussion}

\vspace{-2em}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables}
\begin{tabular}{l 
>{\centering\arraybackslash}p{0.2\linewidth} 
>{\centering\arraybackslash}p{0.2\linewidth} 
>{\centering\arraybackslash}p{0.2\linewidth} 
>{\centering\arraybackslash}p{0.2\linewidth}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{v3Spread}$ & $\log\textsf{cfv2Spread}$ & $\log\textsf{v3S/cfv2S}$ & $\log\textsf{TVL}$ \\
\midrule
% const & 1.383$^{***}$ & 3.016$^{***}$ & -1.633$^{***}$ & 15.257$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ & 0.178$^{}$ & 0.083$^{}$ & 0.095$^{**}$ & -0.083$^{}$ \\
& (0.126) & (0.120) & (0.047) & (0.120) \\
 \textsf{LogReturns} & -0.033$^{***}$ & -0.009$^{}$ & -0.024$^{***}$ & 0.009$^{}$ \\
& (0.008) & (0.006) & (0.006) & (0.006) \\
 \textsf{Volatility} & 0.379$^{***}$ & 0.089$^{**}$ & 0.290$^{***}$ & -0.089$^{**}$ \\
& (0.052) & (0.045) & (0.026) & (0.045) \\
 $\log\textsf{FeeRevenue}$ & -0.869$^{***}$ & -0.201$^{**}$ & -0.668$^{***}$ & 0.201$^{**}$ \\
& (0.119) & (0.079) & (0.079) & (0.079) \\
 \textsf{Markout} & -0.088$^{***}$ & -0.169$^{***}$ & 0.081$^{***}$ & 0.169$^{***}$ \\
& (0.026) & (0.019) & (0.020) & (0.019) \\
 \textsf{CompetitorShare} & 0.222$^{***}$ & 0.088$^{}$ & 0.134$^{***}$ & -0.088$^{}$ \\
& (0.065) & (0.056) & (0.031) & (0.056) \\
 \textsf{Internalization} & 0.062$^{}$ & 0.113$^{***}$ & -0.051$^{}$ & -0.113$^{***}$ \\
& (0.082) & (0.027) & (0.070) & (0.027) \\
\hline \\[-1.8ex]
 Observations & 38440 & 38440 & 38440 & 38440 \\
 N. of groups & 40 & 40 & 40 & 40 \\
 $R^2$ & 0.327 & 0.093 & 0.447 & 0.093 \\
\bottomrule \\[-2.25ex]
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01}
\end{tabular}
\label{table:private-all}
\end{table}

% \begin{table}[H] \centering
% \caption{
% Model (\ref{equation4}) with External Liquidity Variables (All Aggregators)
% }
% \begin{tabular}{l 
% >{\centering\arraybackslash}p{2.5cm} 
% >{\centering\arraybackslash}p{2.5cm} 
% >{\centering\arraybackslash}p{2.5cm} 
% >{\centering\arraybackslash}p{2.5cm}}
% \toprule
% & (1) & (2) & (3) & (4) \\
% & $\log\textsf{v3Spread}$ & $\log\textsf{cfv2Spread}$ & $\log\textsf{v3S/cfv2S}$ & $\log\textsf{TVL}$ \\
% \midrule
% % const & 1.383$^{***}$ & 3.016$^{***}$ & -1.633$^{***}$ & 15.257$^{***}$ \\
% % & (0.000) & (0.000) & (0.000) & (0.000) \\
%  gas price & 0.178$^{}$ & 0.083$^{}$ & 0.095$^{**}$ & -0.083$^{}$ \\
% & (0.126) & (0.120) & (0.047) & (0.120) \\
%  logreturns & -0.033$^{***}$ & -0.009$^{}$ & -0.024$^{***}$ & 0.009$^{}$ \\
% & (0.008) & (0.006) & (0.006) & (0.006) \\
%  volatility & 0.379$^{***}$ & 0.089$^{**}$ & 0.290$^{***}$ & -0.089$^{**}$ \\
% & (0.052) & (0.045) & (0.026) & (0.045) \\
%  fee revenue & -0.869$^{***}$ & -0.201$^{**}$ & -0.668$^{***}$ & 0.201$^{**}$ \\
% & (0.119) & (0.079) & (0.079) & (0.079) \\
%  markout & -0.088$^{***}$ & -0.169$^{***}$ & 0.081$^{***}$ & 0.169$^{***}$ \\
% & (0.026) & (0.019) & (0.020) & (0.019) \\
%  competitor share & 0.222$^{***}$ & 0.088$^{}$ & 0.134$^{***}$ & -0.088$^{}$ \\
% & (0.065) & (0.056) & (0.031) & (0.056) \\
%  internalization & 0.062$^{}$ & 0.113$^{***}$ & -0.051$^{}$ & -0.113$^{***}$ \\
% & (0.082) & (0.027) & (0.070) & (0.027) \\
% \hline \\[-1.8ex]
%  Observations & 38440 & 38440 & 38440 & 38440 \\
%  N. of groups & 40 & 40 & 40 & 40 \\
%  $R^2$ & 0.327 & 0.093 & 0.447 & 0.093 \\
% \bottomrule \\[-2.25ex]
% \multicolumn{5}{l}{\small Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
% \textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01}
% \end{tabular}
% \label{table:private-allx}
% \end{table}

\vspace{-1em}

\autoref{table:private-all} displays the estimation results of each dependent variable using the extended model that includes the competitor trading volume share and internalization ratios.
We find that a higher competitor share of the token pair predicts higher effective spreads, while there is no significant explanatory power from internalization.
Interestingly, the channels in which competitor share and internalization affect market depth differ: the former affects liquidity via concentration while the latter affects liquidity through value locked.

One possible explanation for this difference is that while providing liquidity privately and to competing DEXs are both alternative opportunities for LPs to earn fee revenue, providing liquidity privately is more discretionary, as PMMs can choose which orders to fill, while providing liquidity to a competing DEX requires the LP to take the opposite position of all trades routed to the DEX.
The greater risk involved in this option incentivizes LPs to widen price ranges, following the same intuition as the discussion on volatility and markout. 
Conversely, the lesser risks involved in being a PMM mean that LPs choosing this option may not need to widen ranges on existing position, instead directly withdrawing liquidity from pools to serve as private liquidity.

% Competitor share affects both channels contributing to the overall v3 spread significantly, with higher competitor share predicting lower value locked and lower concentration.
% One potential implication is that LPs may migrate capital from one DEX to another, rather than deploy more capital on other DEXs, to capture fee revenue opportunities on other DEXs created by increased volume share.
% While the work of \cite{huzhang2024competition} shows that competition among centralized cryptocurrency exchanges has a complementary effect on CEXs, our findings show that competition between DEXs for liquidity is more zero-sum in nature.

% Overall v3 spread and counterfactual v2 spread increase in the internalization ratio while the coefficient on concentration is insignificant. 
% The normalized effect size of internalization on v3 spread by all aggregators is larger than that of internalization by UniswapX only.
% A common intuition is that private market makers on these DEX aggregators are typically more sophisticated and better able to detect toxic order flow compared to their counterparts on liquidity pools, with \cite{bachu2024quantifying} supporting this. 
% This lead to uninformed order flow being filled by private liquidity while more toxic flow is left to AMM liquidity pools.
% However, even after controlling for order flow toxicity via the markout variable, higher internalization rates predicts worsening spreads and value locked. 
% Interestingly, internalization rate does not significantly affect the liquidity concentration. 
% This suggests that more internalization of order flow affects passive LPs more adversely than or equally compared to active LPs. 
% Active LPs may be able to adopt strategies for liquidity provision that are insensitive to swaps being routed away to private market makers, whilst passive LPs cannot adequately compete with fillers and active LPs for order flow.



% \begin{table}[h] \centering
% \caption{
% Model (\ref{equation4}) with External Liquidity Variables (UniswapX Only)
% }
% \begin{tabular}{l 
% >{\centering\arraybackslash}p{2.5cm} 
% >{\centering\arraybackslash}p{2.5cm} 
% >{\centering\arraybackslash}p{2.5cm} 
% >{\centering\arraybackslash}p{2.5cm}}

% \toprule
%  & (1) & (2) & (3) & (4) \\
% & $\log\textsf{v3Spread}$ & $\log\textsf{cfv2Spread}$ & $\log\textsf{v3S/cfv2S}$ & $\log\textsf{TVL}$ \\
% \midrule
% % const & 1.383$^{***}$ & 3.016$^{***}$ & -1.633$^{***}$ & 15.257$^{***}$ \\
% % & (0.000) & (0.000) & (0.000) & (0.000) \\
%  $\log\textsf{GasPrice}$ & 0.073$^{*}$ & 0.026$^{}$ & 0.047$^{***}$ & -0.026$^{}$ \\
% & (0.038) & (0.040) & (0.014) & (0.040) \\
%  \textsf{LogReturns} & -0.035$^{***}$ & -0.008$^{}$ & -0.027$^{***}$ & 0.008$^{}$ \\
% & (0.011) & (0.006) & (0.008) & (0.006) \\
%  \textsf{Volatility} & 0.353$^{***}$ & 0.036$^{}$ & 0.317$^{***}$ & -0.036$^{}$ \\
% & (0.081) & (0.064) & (0.048) & (0.064) \\
%  $\log\textsf{FeeRevenue}$ & -0.967$^{***}$ & -0.194$^{**}$ & -0.773$^{***}$ & 0.194$^{**}$ \\
% & (0.108) & (0.084) & (0.051) & (0.084) \\
%  \textsf{Markout} & -0.097$^{***}$ & -0.168$^{***}$ & 0.071$^{***}$ & 0.168$^{***}$ \\
% & (0.021) & (0.027) & (0.026) & (0.027) \\
%  \textsf{CompetitorShare} &  0.222$^{***}$ & 0.115$^{*}$ & 0.107$^{***}$ & -0.115$^{*}$ \\
% & (0.062) & (0.068) & (0.028) & (0.068) \\
%  \textsf{Internalization} & 0.051$^{**}$ & 0.050$^{***}$ & 0.001$^{}$ & -0.050$^{***}$ \\
% & (0.020) & (0.019) & (0.006) & (0.019) \\
% \hline \\[-1.8ex]
%  Observations & 37081 & 37081 & 37081 & 37081 \\
%  N. of groups & 36 & 36 & 36 & 36 \\
%  $R^2$ & 0.364 & 0.082 & 0.545 & 0.082 \\
% \bottomrule \\[-2.25ex]
% \multicolumn{5}{l}{\small Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
% \textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01}
% \end{tabular}
% \label{table:private-unix}
% \end{table}

% \paragraph{Robustness Checks.}
% %We conduct a variety of robustness checks for our findings, and display the regression tables in the Appendix. 
% %These include changing pool FE to chain FE, adjusting the horizon for log-returns and markouts, computing effective spreads with different trade sizes, analyzing the full sample with outliers and sub-samples, and predicting future liquidity at longer time horizons.
% %Main results holds with all robustness checks.

% We conduct a variety of robustness checks to validate our findings, with regression tables presented in the Appendix~\ref{appendix:robust}. 
% These checks include varying the horizons for log-returns and markouts, calculating effective spreads across different trade sizes, analyzing the full sample with outliers and subsamples, and predicting future liquidity over extended time horizons. 
% The main results remain robust across all checks.

% $\log\textsf{GasPrice}$
% \textsf{LogReturns}
% \textsf{Volatility}
% $\log\textsf{FeeRevenue}$
% \textsf{Markout}
% \textsf{Internalization}
% $\mathcal{A}=\textsf{\{1in,CoW,UniX\}}$






% Splits: WETH-Stable and WETH-Nonstable; L1 pools and L2 pools; 5 bps pools and 30 bps pools
% 40777, 40751

==> sections/OldA.tex <==
\section{Summary Statistics}
% \label{appendix:summarystat}

\setlength{\tabcolsep}{0.5em} % for the horizontal padding
\renewcommand{\arraystretch}{1.25}% for the vertical padding

\subsection{Liquidity Metrics}

Tables \ref{tab:ssall}, \ref{tab:sseth}, and \ref{tab:ssl2} display summary statistics for liqudity metrics used in our analysis over all sample pools, Ethereum pools only, and L2 pools only. While Ethereum pools have better liquidity (lower overall effective spread and higher TVL) than L2 pools, concentration is better in L2 pools. Additionally, liquidity in L2 pools is more volatile than liquidity in Ethereum pools. Figure \ref{fig:histogram} visualizes this trend for the effective spread.


\begin{figure}[H]
    \centering
    \includegraphics[scale=0.6]{plots/WDL-histogram.pdf}
    \caption{\centering Histogram of effective spread (when trading 1 WETH) on all  liquidity pools in the sample.}
    \label{fig:histogram}
\end{figure}

\begin{table}[H]
    \centering
    \begin{tabular}{ccccc}
\toprule
 & $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
$N$ & 37081 & 37081 & 37081 & 37081 \\
Mean & 1.3856 & 3.0190 & -1.6334 & 15.2538 \\
S.D. & 2.6157 & 2.7188 & 1.1333 & 2.6930 \\
25\% & -0.7753 & 0.9417 & -2.3772 & 13.2810 \\
50\% & 1.2918 & 3.0863 & -1.7305 & 15.1991 \\
75\% & 3.2006 & 5.0173 & -0.9160 & 17.3153 \\
\bottomrule
\end{tabular}
\vspace{0.5em}
    \caption{Summary Statistics, Liquidity Metrics, All Pools.}
    \label{tab:ssall}
\end{table}

\begin{table}[H]
    \centering
    \begin{tabular}{ccccc}
\toprule
 & $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
$N$ & 11798 & 11798 & 11798 & 11798 \\
Mean & -0.8179 & 0.1433 & -0.9613 & 18.1686 \\
S.D. & 1.7341 & 1.5084 & 0.9754 & 1.4190 \\
25\% & -1.9108 & -0.9863 & -1.6462 & 17.3567 \\
50\% & -1.2367 & -0.0039 & -0.9490 & 18.3497 \\
75\% & -0.0904 & 1.0277 & -0.2764 & 19.4486 \\
\bottomrule
\end{tabular}
\vspace{0.5em}
    \caption{Summary Statistics, Liquidity Metrics, Ethereum Pools Only.}
    \label{tab:sseth}
\end{table}

\vspace{-5em}

\begin{table}[H]
    \centering
    \begin{tabular}{ccccc}
\toprule
 & $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
$N$ & 25283 & 25283 & 25283 & 25283 \\
Mean & 2.4138 & 4.3609 & -1.9471 & 13.8936 \\
std & 2.3041 & 2.0297 & 1.0633 & 1.9704 \\
25\% & 0.8158 & 2.8413 & -2.5429 & 12.5303 \\
50\% & 2.2676 & 4.3111 & -2.0090 & 13.9946 \\
75\% & 3.8945 & 5.7274 & -1.3756 & 15.3733 \\
\bottomrule
\end{tabular}
\vspace{0.5em}
    \caption{Summary Statistics, Liquidity Metrics, L2 Pools Only.}
    \label{tab:ssl2}
\end{table}

Figure \ref{fig:liquidity1} plots time series for effective spread and TVL for fixed pairs and fees on varying blockchains. Upon a pool's creation, liquidity tends to ``rush'' into a pool, with spread plummeting and TVL skyrocketing, before stabilizing around a certain level with smaller deviations later on. There appears to be moderate comovement in spread and TVL between blockchains for a given pair and fee tier. Figure \ref{fig:liquidity2} shows similar plots, this time fixing the blockchain and looking at various token pairs.


Figures \ref{fig:liquidity3} compares effective spreads with counterfactual v2 spreads. For most pools, such as the one depicted the left, the v3 spread is almost always lower than the counterfactual v2 spread, suggesting that liquidity is usually well-concentrated. However, for some pools, such as that in the right there are sustained periods when the counterfactual v2 spread is lower than the v3 spread, implying poor concentration of liquidity for a prolonged amount of time.

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.35]{plots/WDL-v3v2-1.pdf} \includegraphics[scale=0.35]{plots/WDL-v3v2-2.pdf}
    \caption{\centering Time series for effective spread and counterfactual v2 spread for the selected liquidity pools.}
    \label{fig:liquidity3}
\end{figure}



\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{plots/WDL-liquidity-WETH-USDC.pdf} \\[0.5\baselineskip]
    \includegraphics[scale=0.5]{plots/WDL-liquidity-WETH-WBTC.pdf}
    \caption{\centering Time series for effective spread (when trading 1 WETH) and TVL on selected liquidity pools.}
    \label{fig:liquidity1}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{plots/WDL-liquidity-ethereum.pdf} \\[0.5\baselineskip]
    \includegraphics[scale=0.5]{plots/WDL-liquidity-polygon.pdf}
    \caption{\centering Time series for effective spread (when trading 1 WETH) and TVL on selected liquidity pools.}
    \label{fig:liquidity2}
\end{figure}

\subsection{Independent Variables}

\begin{table}[H]
    \centering
    \begin{tabular}{cccccc}
\toprule
 & $\log\textsf{GasPrice}$ & \textsf{LogReturns} & \textsf{Volatility} & $\log\textsf{FeeRevenue}$ & \textsf{Markout} \\ 
\midrule
$N$ & 37081 & 37081 & 37081 & 37081 & 37081 \\
Mean & 1.8741 & -0.0045 & 4.9747 & -7.8960 & -0.0011 \\
S.D. & 5.0924 & 3.3101 & 4.0251 & 1.3687 & 0.0078 \\
25\% & -0.8640 & -1.3436 & 2.7120 & -8.7129 & -0.0007 \\
50\% & 3.1149 & 0.0183 & 4.1178 & -7.8482 & -0.0003 \\
75\% & 4.4568 & 1.5362 & 6.0260 & -7.0140 & -0.0001 \\
\bottomrule
\end{tabular}
\vspace{0.5em}
    \caption{Summary Statistics, Baseline Model.}
    \label{tab:my_label1}
\end{table}

\vspace{-2em}

\begin{table}[H]
    \centering
    \begin{tabular}{cccc}
\toprule
 & \textsf{Competition} & \makecell{\textsf{Internalization} \\ (all aggregators)} & \makecell{\textsf{Internalization} \\ (UniswapX only)} \\
\midrule
$N$ & 37081 & 37081 & 3899 \\
Mean & 0.2563 & 0.0510 & 0.0130 \\
S.D. & 0.2511 & 0.1189 & 0.0241 \\
25\% & 0.0648 & 0.0007 & 0.0009 \\
50\% & 0.1694 & 0.0057 & 0.0059 \\
75\% & 0.3622 & 0.0353 & 0.0145 \\
\bottomrule
\end{tabular}

\vspace{0.5em}
    \caption{\centering Summary Statistics, External Liquidity Variables Model. \\[0.25\baselineskip] }
    \label{tab:my_label2}
\end{table}

Table \ref{tab:my_label1} displays summary statistics for independent variables in the baseline model, and Table \ref{tab:my_label2} does the same for the DEX competition ratio and internalization ratio (using all aggregators and only UniswapX). As UniswapX was launched on July 17, 2023 on the Ethereum Mainnet, summary statistics for the internalization ratio with respect to UniswapX alone only include Ethereum pool-days after the launch date.


==> sections/OldB.tex <==
\section{Robustness Checks}
% \label{appendix:robust}

\renewcommand{\arraystretch}{1}% for the vertical padding

% \subsection{Chain and Day Fixed Effects}

% \begin{table}[H] \centering
% \caption{
% Baseline Regression Model (\ref{equation1}) with Decomposition (\ref{equation2}) $+$ (\ref{equation3})
% }
% \resizebox{0.85\textwidth}{!}{%
% \begin{tabular}{l 
% >{\centering\arraybackslash}p{2.3cm} 
% >{\centering\arraybackslash}p{2.3cm} 
% >{\centering\arraybackslash}p{2.3cm} 
% >{\centering\arraybackslash}p{2.3cm}}
% \toprule
% & (1) & (2) & (3) & (4) \\
% & $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
% \midrule
% % const & 1.383$^{***}$ & 3.016$^{***}$ & -1.633$^{***}$ & 15.257$^{***}$ \\
% % & (0.000) & (0.000) & (0.000) & (0.000) \\
%  $\log\textsf{GasPrice}$ &  0.082$^{***}$ & 0.033$^{}$ & 0.050$^{***}$ & -0.033$^{}$ \\
% & (0.016) & (0.020) & (0.012) & (0.020) \\
%  \textsf{LogReturns} & 0.080$^{***}$ & 0.071$^{***}$ & 0.009$^{}$ & -0.071$^{***}$ \\
% & (0.018) & (0.007) & (0.011) & (0.007) \\
%  \textsf{Volatility} & 1.639$^{***}$ & 0.926$^{***}$ & 0.713$^{***}$ & -0.926$^{***}$ \\
% & (0.335) & (0.262) & (0.103) & (0.262) \\
%  $\log\textsf{FeeRevenue}$ &  -1.177$^{***}$ & -0.379$^{*}$ & -0.798$^{***}$ & 0.379$^{*}$ \\
% & (0.235) & (0.229) & (0.041) & (0.229) \\
%  \textsf{Markout} & -0.129$^{***}$ & -0.213$^{***}$ & 0.084$^{***}$ & 0.213$^{***}$ \\
% & (0.040) & (0.046) & (0.009) & (0.046) \\
% \midrule
%  Observations & 37081 & 37081 & 37081 & 37081 \\
%  N. of groups & 4 & 4 & 4 & 4 \\
%  $R^2$ & 0.228 & 0.071 & 0.485 & 0.071 \\
% \bottomrule
% \multicolumn{5}{l}{Chain and day fixed effects are included; standard errors are clustered at the pool level.} \\
% \textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} 
% \end{tabular}%
% }
% \label{table:baseline}
% \end{table}

% \begin{table}[htb] \centering
% \caption{
% Model (\ref{equation4}) with External Liquidity Variables (All Aggregators)
% }
% \resizebox{0.85\textwidth}{!}{%
% \begin{tabular}{l 
% >{\centering\arraybackslash}p{2.3cm} 
% >{\centering\arraybackslash}p{2.3cm} 
% >{\centering\arraybackslash}p{2.3cm} 
% >{\centering\arraybackslash}p{2.3cm}}
% \toprule
% & (1) & (2) & (3) & (4) \\
% & $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
% \midrule
% % const & 1.383$^{***}$ & 3.016$^{***}$ & -1.633$^{***}$ & 15.257$^{***}$ \\
% % & (0.000) & (0.000) & (0.000) & (0.000) \\
%  $\log\textsf{GasPrice}$ &  0.105$^{***}$ & 0.054$^{**}$ & 0.051$^{***}$ & -0.054$^{**}$ \\
% & (0.023) & (0.027) & (0.011) & (0.027) \\
%  \textsf{LogReturns} & 0.033$^{***}$ & 0.030$^{***}$ & 0.003$^{}$ & -0.030$^{***}$ \\
% & (0.008) & (0.005) & (0.011) & (0.005) \\
%  \textsf{Volatility} & 1.083$^{***}$ & 0.441$^{**}$ & 0.642$^{***}$ & -0.441$^{**}$ \\
% & (0.273) & (0.222) & (0.102) & (0.222) \\
%  $\log\textsf{FeeRevenue}$ &  -0.926$^{***}$ & -0.159$^{}$ & -0.767$^{***}$ & 0.159$^{}$ \\
% & (0.189) & (0.203) & (0.034) & (0.203) \\
%  \textsf{Markout} & -0.124$^{***}$ & -0.209$^{***}$ & 0.085$^{***}$ & 0.209$^{***}$ \\
% & (0.035) & (0.041) & (0.009) & (0.041) \\
%  \textsf{Competition} & 0.677$^{***}$ & 0.586$^{***}$ & 0.091$^{***}$ & -0.586$^{***}$ \\
% & (0.144) & (0.153) & (0.013) & (0.153) \\
%  \textsf{Internalization} & 0.667$^{***}$ & 0.593$^{***}$ & 0.073$^{***}$ & -0.593$^{***}$ \\
% & (0.108) & (0.101) & (0.020) & (0.101) \\
% \midrule
%  Observations & 37081 & 37081 & 37081 & 37081 \\
%  N. of groups & 4 & 4 & 4 & 4 \\
%  $R^2$ & 0.434 & 0.310 & 0.501 & 0.310 \\
% \bottomrule \\
% \multicolumn{5}{l}{Chain and day fixed effects are included; standard errors are clustered at the pool level.} \\
% \textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
% \end{tabular}%
% }
% \label{table:baseline}
% \end{table}

% \begin{table}[H] \centering
% \caption{
% Model (\ref{equation4}) with External Liquidity Variables (UniswapX Only)
% }
% \resizebox{0.85\textwidth}{!}{%
% \begin{tabular}{l 
% >{\centering\arraybackslash}p{2.3cm} 
% >{\centering\arraybackslash}p{2.3cm} 
% >{\centering\arraybackslash}p{2.3cm} 
% >{\centering\arraybackslash}p{2.3cm}}
% \toprule
% & (1) & (2) & (3) & (4) \\
% & $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
% \midrule
% % const & 1.383$^{***}$ & 3.016$^{***}$ & -1.633$^{***}$ & 15.257$^{***}$ \\
% % & (0.000) & (0.000) & (0.000) & (0.000) \\
%  $\log\textsf{GasPrice}$ &  0.037$^{}$ & -0.007$^{}$ & 0.044$^{***}$ & 0.007$^{}$ \\
% & (0.022) & (0.030) & (0.009) & (0.030) \\
%  \textsf{LogReturns} & 0.044$^{***}$ & 0.040$^{***}$ & 0.004$^{}$ & -0.040$^{***}$ \\
% & (0.009) & (0.004) & (0.011) & (0.004) \\
%  \textsf{Volatility} & 1.126$^{***}$ & 0.479$^{**}$ & 0.647$^{***}$ & -0.479$^{**}$ \\
% & (0.288) & (0.243) & (0.099) & (0.243) \\
%  $\log\textsf{FeeRevenue}$ &  -0.950$^{***}$ & -0.181$^{}$ & -0.769$^{***}$ & 0.181$^{}$ \\
% & (0.211) & (0.219) & (0.038) & (0.219) \\
%  \textsf{Markout} & -0.135$^{***}$ & -0.219$^{***}$ & 0.083$^{***}$ & 0.219$^{***}$ \\
% & (0.040) & (0.047) & (0.008) & (0.047) \\
%  \textsf{Competition} & 0.849$^{***}$ & 0.739$^{***}$ & 0.110$^{***}$ & -0.739$^{***}$ \\
% & (0.135) & (0.137) & (0.020) & (0.137) \\
%  \textsf{Internalization} & 0.127$^{***}$ & 0.114$^{***}$ & 0.014$^{***}$ & -0.114$^{***}$ \\
% & (0.015) & (0.016) & (0.005) & (0.016) \\
% \midrule
%  Observations & 37081 & 37081 & 37081 & 37081 \\
%  N. of groups & 4 & 4 & 4 & 4 \\
%  $R^2$ & 0.344 & 0.203 & 0.495 & 0.203 \\
% \bottomrule \\
% \multicolumn{5}{l}{Chain and day fixed effects are included; standard errors are clustered at the pool level.} \\
% \textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
% \end{tabular}%
% }
% \label{table:baseline}
% \end{table}

\subsection{Return and Markout Horizons}

\paragraph{Weekly Returns} \text{}

\begin{table}[H] \centering
\caption{
Baseline Regression Model (\ref{equation1}) with Decomposition (\ref{equation2}) $+$ (\ref{equation3})
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.383$^{***}$ & 3.016$^{***}$ & -1.633$^{***}$ & 15.257$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.085$^{**}$ & 0.032$^{}$ & 0.053$^{***}$ & -0.032$^{}$ \\
& (0.041) & (0.042) & (0.014) & (0.042) \\
 \textsf{LogReturns} & -0.047$^{**}$ & -0.025$^{}$ & -0.021$^{}$ & 0.025$^{}$ \\
& (0.021) & (0.016) & (0.014) & (0.016) \\
 \textsf{Volatility} & 0.352$^{***}$ & 0.032$^{}$ & 0.320$^{***}$ & -0.032$^{}$ \\
& (0.084) & (0.064) & (0.051) & (0.064) \\
 $\log\textsf{FeeRevenue}$ &  -1.026$^{***}$ & -0.227$^{***}$ & -0.799$^{***}$ & 0.227$^{***}$ \\
& (0.102) & (0.080) & (0.050) & (0.080) \\
 \textsf{Markout} & -0.095$^{***}$ & -0.168$^{***}$ & 0.073$^{***}$ & 0.168$^{***}$ \\
& (0.021) & (0.027) & (0.027) & (0.027) \\
\midrule
 Observations & 37081 & 37081 & 37081 & 37081 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.350 & 0.071 & 0.537 & 0.071 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} 
\end{tabular}%
}
\label{table:baseline}
\end{table}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (All Aggregators)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.383$^{***}$ & 3.016$^{***}$ & -1.633$^{***}$ & 15.257$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.087$^{**}$ & 0.037$^{}$ & 0.050$^{***}$ & -0.038$^{}$ \\
& (0.037) & (0.038) & (0.014) & (0.038) \\
 \textsf{LogReturns} & -0.049$^{**}$ & -0.027$^{*}$ & -0.022$^{}$ & 0.027$^{*}$ \\
& (0.021) & (0.016) & (0.014) & (0.016) \\
 \textsf{Volatility} & 0.336$^{***}$ & 0.024$^{}$ & 0.311$^{***}$ & -0.024$^{}$ \\
& (0.079) & (0.062) & (0.052) & (0.062) \\
 $\log\textsf{FeeRevenue}$ &  -0.959$^{***}$ & -0.188$^{**}$ & -0.770$^{***}$ & 0.188$^{**}$ \\
& (0.106) & (0.083) & (0.051) & (0.083) \\
 \textsf{Markout} & -0.098$^{***}$ & -0.169$^{***}$ & 0.071$^{***}$ & 0.169$^{***}$ \\
& (0.021) & (0.028) & (0.026) & (0.028) \\
 \textsf{Competition} & 0.227$^{***}$ & 0.118$^{*}$ & 0.109$^{***}$ & -0.118$^{*}$ \\
& (0.061) & (0.066) & (0.028) & (0.066) \\
 \textsf{Internalization} & 0.166$^{***}$ & 0.135$^{***}$ & 0.031$^{}$ & -0.135$^{***}$ \\
& (0.051) & (0.033) & (0.026) & (0.033) \\
\midrule
 Observations & 37081 & 37081 & 37081 & 37081 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.375 & 0.096 & 0.545 & 0.096 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (UniswapX Only)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.383$^{***}$ & 3.016$^{***}$ & -1.633$^{***}$ & 15.257$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.073$^{*}$ & 0.026$^{}$ & 0.047$^{***}$ & -0.026$^{}$ \\
& (0.038) & (0.040) & (0.014) & (0.040) \\
 \textsf{LogReturns} & -0.046$^{**}$ & -0.025$^{}$ & -0.021$^{}$ & 0.025$^{}$ \\
& (0.021) & (0.016) & (0.014) & (0.016) \\
 \textsf{Volatility} & 0.334$^{***}$ & 0.023$^{}$ & 0.311$^{***}$ & -0.023$^{}$ \\
& (0.082) & (0.063) & (0.052) & (0.063) \\
 $\log\textsf{FeeRevenue}$ &  -0.969$^{***}$ & -0.195$^{**}$ & -0.773$^{***}$ & 0.195$^{**}$ \\
& (0.109) & (0.084) & (0.051) & (0.084) \\
 \textsf{Markout} & -0.097$^{***}$ & -0.168$^{***}$ & 0.071$^{***}$ & 0.168$^{***}$ \\
& (0.021) & (0.027) & (0.026) & (0.027) \\
 \textsf{Competition} & 0.222$^{***}$ & 0.115$^{*}$ & 0.107$^{***}$ & -0.115$^{*}$ \\
& (0.062) & (0.068) & (0.028) & (0.068) \\
 \textsf{Internalization} & 0.051$^{**}$ & 0.050$^{***}$ & 0.001$^{}$ & -0.050$^{***}$ \\
& (0.020) & (0.019) & (0.007) & (0.019) \\
\midrule
 Observations & 37081 & 37081 & 37081 & 37081 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.365 & 0.082 & 0.544 & 0.082 \\
\bottomrule 
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\paragraph{Hourly Markout} \text{}

\begin{table}[H] \centering
\caption{
Baseline Regression Model (\ref{equation1}) with Decomposition (\ref{equation2}) $+$ (\ref{equation3})
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.384$^{***}$ & 3.018$^{***}$ & -1.634$^{***}$ & 15.255$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.083$^{**}$ & 0.029$^{}$ & 0.054$^{***}$ & -0.029$^{}$ \\
& (0.041) & (0.043) & (0.014) & (0.043) \\
 \textsf{LogReturns} & -0.036$^{***}$ & -0.009$^{}$ & -0.027$^{***}$ & 0.009$^{}$ \\
& (0.010) & (0.006) & (0.008) & (0.006) \\
 \textsf{Volatility} & 0.371$^{***}$ & 0.046$^{}$ & 0.325$^{***}$ & -0.046$^{}$ \\
& (0.082) & (0.065) & (0.048) & (0.065) \\
 $\log\textsf{FeeRevenue}$ &  -1.015$^{***}$ & -0.210$^{**}$ & -0.805$^{***}$ & 0.210$^{**}$ \\
& (0.102) & (0.083) & (0.051) & (0.083) \\
 markout 1hr & -0.081$^{***}$ & -0.151$^{***}$ & 0.070$^{***}$ & 0.151$^{***}$ \\
& (0.018) & (0.017) & (0.017) & (0.017) \\
\midrule
 Observations & 37090 & 37090 & 37090 & 37090 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.345 & 0.060 & 0.539 & 0.060 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} 
\end{tabular}%
}
\label{table:baseline}
\end{table}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (All Aggregators)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.384$^{***}$ & 3.018$^{***}$ & -1.634$^{***}$ & 15.255$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.085$^{**}$ & 0.035$^{}$ & 0.050$^{***}$ & -0.035$^{}$ \\
& (0.037) & (0.039) & (0.014) & (0.039) \\
 \textsf{LogReturns} & -0.036$^{***}$ & -0.009$^{}$ & -0.027$^{***}$ & 0.009$^{}$ \\
& (0.011) & (0.006) & (0.008) & (0.006) \\
 \textsf{Volatility} & 0.356$^{***}$ & 0.040$^{}$ & 0.316$^{***}$ & -0.040$^{}$ \\
& (0.076) & (0.063) & (0.048) & (0.063) \\
 $\log\textsf{FeeRevenue}$ &  -0.947$^{***}$ & -0.171$^{**}$ & -0.776$^{***}$ & 0.171$^{**}$ \\
& (0.107) & (0.085) & (0.051) & (0.085) \\
 markout 1hr & -0.082$^{***}$ & -0.151$^{***}$ & 0.069$^{***}$ & 0.151$^{***}$ \\
& (0.017) & (0.017) & (0.016) & (0.017) \\
 \textsf{Competition} & 0.227$^{***}$ & 0.116$^{*}$ & 0.110$^{***}$ & -0.116$^{*}$ \\
& (0.061) & (0.068) & (0.029) & (0.068) \\
 \textsf{Internalization} & 0.167$^{***}$ & 0.136$^{***}$ & 0.031$^{}$ & -0.136$^{***}$ \\
& (0.051) & (0.033) & (0.026) & (0.033) \\
\midrule
 Observations & 37090 & 37090 & 37090 & 37090 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.371 & 0.085 & 0.547 & 0.085 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (UniswapX Only)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.384$^{***}$ & 3.018$^{***}$ & -1.634$^{***}$ & 15.255$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.071$^{*}$ & 0.024$^{}$ & 0.048$^{***}$ & -0.024$^{}$ \\
& (0.039) & (0.041) & (0.014) & (0.041) \\
 \textsf{LogReturns} & -0.034$^{***}$ & -0.007$^{}$ & -0.027$^{***}$ & 0.007$^{}$ \\
& (0.011) & (0.006) & (0.008) & (0.006) \\
 \textsf{Volatility} & 0.353$^{***}$ & 0.037$^{}$ & 0.316$^{***}$ & -0.037$^{}$ \\
& (0.080) & (0.065) & (0.048) & (0.065) \\
 $\log\textsf{FeeRevenue}$ &  -0.957$^{***}$ & -0.178$^{**}$ & -0.778$^{***}$ & 0.178$^{**}$ \\
& (0.110) & (0.086) & (0.052) & (0.086) \\
 markout 1hr & -0.082$^{***}$ & -0.151$^{***}$ & 0.069$^{***}$ & 0.151$^{***}$ \\
& (0.017) & (0.017) & (0.016) & (0.017) \\
 \textsf{Competition} & 0.221$^{***}$ & 0.114$^{*}$ & 0.108$^{***}$ & -0.114$^{*}$ \\
& (0.063) & (0.069) & (0.028) & (0.069) \\
 \textsf{Internalization} & 0.052$^{**}$ & 0.051$^{***}$ & 0.001$^{}$ & -0.051$^{***}$ \\
& (0.020) & (0.020) & (0.007) & (0.020) \\
\midrule
 Observations & 37090 & 37090 & 37090 & 37090 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.360 & 0.072 & 0.546 & 0.072 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\clearpage
\subsection{Smaller and Larger Trade Size}

\paragraph{0.1 WETH Trade Size} \text{}

\begin{table}[H] \centering
\caption{
Baseline Regression Model (\ref{equation1}) with Decomposition (\ref{equation2}) $+$ (\ref{equation3})
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & -0.492$^{***}$ & 0.774$^{***}$ & -1.266$^{***}$ & 15.200$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.064$^{}$ & 0.020$^{}$ & 0.043$^{***}$ & -0.021$^{}$ \\
& (0.043) & (0.045) & (0.013) & (0.045) \\
 \textsf{LogReturns} & -0.035$^{***}$ & -0.008$^{}$ & -0.027$^{***}$ & 0.008$^{}$ \\
& (0.010) & (0.006) & (0.009) & (0.006) \\
 \textsf{Volatility} & 0.415$^{***}$ & 0.078$^{}$ & 0.336$^{***}$ & -0.078$^{}$ \\
& (0.075) & (0.055) & (0.046) & (0.055) \\
 $\log\textsf{FeeRevenue}$ &  -1.067$^{***}$ & -0.296$^{***}$ & -0.771$^{***}$ & 0.296$^{***}$ \\
& (0.104) & (0.084) & (0.047) & (0.084) \\
 \textsf{Markout} & -0.105$^{***}$ & -0.173$^{***}$ & 0.068$^{**}$ & 0.173$^{***}$ \\
& (0.025) & (0.027) & (0.028) & (0.027) \\
\midrule
 Observations & 37525 & 37525 & 37525 & 37525 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.395 & 0.091 & 0.539 & 0.091 \\
\bottomrule \\
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} 
\end{tabular}%
}
\label{table:baseline}
\end{table}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (All Aggregators)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & -0.492$^{***}$ & 0.774$^{***}$ & -1.266$^{***}$ & 15.200$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.065$^{}$ & 0.027$^{}$ & 0.038$^{***}$ & -0.027$^{}$ \\
& (0.040) & (0.041) & (0.013) & (0.041) \\
 \textsf{LogReturns} & -0.035$^{***}$ & -0.008$^{}$ & -0.027$^{***}$ & 0.008$^{}$ \\
& (0.010) & (0.006) & (0.009) & (0.006) \\
 \textsf{Volatility} & 0.395$^{***}$ & 0.070$^{}$ & 0.326$^{***}$ & -0.070$^{}$ \\
& (0.072) & (0.054) & (0.047) & (0.054) \\
 $\log\textsf{FeeRevenue}$ &  -1.001$^{***}$ & -0.257$^{***}$ & -0.744$^{***}$ & 0.257$^{***}$ \\
& (0.110) & (0.090) & (0.047) & (0.090) \\
 \textsf{Markout} & -0.106$^{***}$ & -0.174$^{***}$ & 0.067$^{**}$ & 0.174$^{***}$ \\
& (0.024) & (0.028) & (0.027) & (0.028) \\
 \textsf{Competition} & 0.221$^{***}$ & 0.113$^{}$ & 0.109$^{***}$ & -0.113$^{}$ \\
& (0.084) & (0.084) & (0.023) & (0.084) \\
 \textsf{Internalization} & 0.146$^{***}$ & 0.138$^{***}$ & 0.008$^{}$ & -0.138$^{***}$ \\
& (0.050) & (0.033) & (0.026) & (0.033) \\
\midrule
 Observations & 37525 & 37525 & 37525 & 37525 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.416 & 0.114 & 0.546 & 0.114 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (UniswapX Only)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & -0.492$^{***}$ & 0.774$^{***}$ & -1.266$^{***}$ & 15.200$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.052$^{}$ & 0.015$^{}$ & 0.037$^{***}$ & -0.015$^{}$ \\
& (0.041) & (0.043) & (0.013) & (0.043) \\
 \textsf{LogReturns} & -0.033$^{***}$ & -0.006$^{}$ & -0.027$^{***}$ & 0.007$^{}$ \\
& (0.010) & (0.006) & (0.009) & (0.006) \\
 \textsf{Volatility} & 0.393$^{***}$ & 0.067$^{}$ & 0.325$^{***}$ & -0.067$^{}$ \\
& (0.075) & (0.056) & (0.047) & (0.056) \\
 $\log\textsf{FeeRevenue}$ &  -1.010$^{***}$ & -0.264$^{***}$ & -0.746$^{***}$ & 0.264$^{***}$ \\
& (0.112) & (0.090) & (0.047) & (0.090) \\
 \textsf{Markout} & -0.106$^{***}$ & -0.173$^{***}$ & 0.067$^{**}$ & 0.173$^{***}$ \\
& (0.024) & (0.027) & (0.027) & (0.027) \\
 \textsf{Competition} & 0.217$^{**}$ & 0.111$^{}$ & 0.107$^{***}$ & -0.111$^{}$ \\
& (0.086) & (0.085) & (0.023) & (0.085) \\
 \textsf{Internalization} & 0.043$^{**}$ & 0.052$^{***}$ & -0.009$^{}$ & -0.052$^{***}$ \\
& (0.019) & (0.020) & (0.008) & (0.020) \\
\midrule
 Observations & 37525 & 37525 & 37525 & 37525 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.408 & 0.101 & 0.546 & 0.101 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\paragraph{10 WETH Trade Size} \text{}

\begin{table}[H] \centering
\caption{
Baseline Regression Model (\ref{equation1}) with Decomposition (\ref{equation2}) $+$ (\ref{equation3})
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 3.246$^{***}$ & 5.084$^{***}$ & -1.838$^{***}$ & 15.490$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.113$^{***}$ & 0.064$^{}$ & 0.049$^{***}$ & -0.064$^{}$ \\
& (0.040) & (0.042) & (0.015) & (0.042) \\
 \textsf{LogReturns} & -0.044$^{***}$ & -0.010$^{*}$ & -0.034$^{***}$ & 0.010$^{*}$ \\
& (0.011) & (0.006) & (0.010) & (0.006) \\
 \textsf{Volatility} & 0.396$^{***}$ & 0.080$^{}$ & 0.316$^{***}$ & -0.080$^{}$ \\
& (0.078) & (0.060) & (0.050) & (0.060) \\
 $\log\textsf{FeeRevenue}$ &  -1.036$^{***}$ & -0.240$^{***}$ & -0.796$^{***}$ & 0.240$^{***}$ \\
& (0.108) & (0.089) & (0.056) & (0.089) \\
 \textsf{Markout} & -0.095$^{***}$ & -0.182$^{***}$ & 0.087$^{***}$ & 0.182$^{***}$ \\
& (0.022) & (0.022) & (0.021) & (0.022) \\
\midrule
 Observations & 34871 & 34871 & 34871 & 34871 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.337 & 0.085 & 0.506 & 0.085 \\
\bottomrule 
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} 
\end{tabular}%
}
\label{table:baseline}
\end{table}

\vspace{-1.25cm}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (All Aggregators)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 3.246$^{***}$ & 5.084$^{***}$ & -1.838$^{***}$ & 15.490$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.099$^{***}$ & 0.059$^{}$ & 0.040$^{**}$ & -0.059$^{}$ \\
& (0.038) & (0.039) & (0.016) & (0.039) \\
 \textsf{LogReturns} & -0.042$^{***}$ & -0.009$^{}$ & -0.033$^{***}$ & 0.009$^{}$ \\
& (0.012) & (0.006) & (0.010) & (0.006) \\
 \textsf{Volatility} & 0.372$^{***}$ & 0.071$^{}$ & 0.301$^{***}$ & -0.071$^{}$ \\
& (0.073) & (0.059) & (0.047) & (0.059) \\
 $\log\textsf{FeeRevenue}$ &  -0.949$^{***}$ & -0.203$^{**}$ & -0.746$^{***}$ & 0.203$^{**}$ \\
& (0.115) & (0.091) & (0.057) & (0.091) \\
 \textsf{Markout} & -0.098$^{***}$ & -0.183$^{***}$ & 0.085$^{***}$ & 0.183$^{***}$ \\
& (0.021) & (0.023) & (0.019) & (0.023) \\
 \textsf{Competition} & 0.225$^{***}$ & 0.082$^{}$ & 0.143$^{***}$ & -0.082$^{}$ \\
& (0.061) & (0.061) & (0.027) & (0.061) \\
 \textsf{Internalization} & 0.208$^{***}$ & 0.110$^{***}$ & 0.097$^{***}$ & -0.110$^{***}$ \\
& (0.037) & (0.028) & (0.021) & (0.028) \\
\midrule
 Observations & 34871 & 34871 & 34871 & 34871 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.361 & 0.096 & 0.523 & 0.096 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (UniswapX Only)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 3.246$^{***}$ & 5.084$^{***}$ & -1.838$^{***}$ & 15.490$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.100$^{***}$ & 0.059$^{}$ & 0.040$^{***}$ & -0.060$^{}$ \\
& (0.038) & (0.039) & (0.016) & (0.039) \\
 \textsf{LogReturns} & -0.041$^{***}$ & -0.008$^{}$ & -0.033$^{***}$ & 0.008$^{}$ \\
& (0.012) & (0.006) & (0.010) & (0.006) \\
 \textsf{Volatility} & 0.377$^{***}$ & 0.074$^{}$ & 0.304$^{***}$ & -0.074$^{}$ \\
& (0.076) & (0.059) & (0.050) & (0.059) \\
 $\log\textsf{FeeRevenue}$ &  -0.978$^{***}$ & -0.216$^{**}$ & -0.762$^{***}$ & 0.216$^{**}$ \\
& (0.113) & (0.089) & (0.057) & (0.089) \\
 \textsf{Markout} & -0.098$^{***}$ & -0.182$^{***}$ & 0.085$^{***}$ & 0.182$^{***}$ \\
& (0.022) & (0.022) & (0.020) & (0.022) \\
 \textsf{Competition} & 0.212$^{***}$ & 0.078$^{}$ & 0.134$^{***}$ & -0.078$^{}$ \\
& (0.062) & (0.061) & (0.028) & (0.061) \\
 \textsf{Internalization} & 0.062$^{***}$ & 0.048$^{**}$ & 0.013$^{}$ & -0.048$^{**}$ \\
& (0.023) & (0.020) & (0.008) & (0.020) \\
\midrule
 Observations & 34871 & 34871 & 34871 & 34871 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.351 & 0.092 & 0.517 & 0.092 \\
\bottomrule \\[-2.25ex]
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\clearpage
\subsection{Full Sample and Split Samples}

\paragraph{Including Markout Outliers} \text{}

\begin{table}[H] \centering
\caption{
Baseline Regression Model (\ref{equation1}) with Decomposition (\ref{equation2}) $+$ (\ref{equation3})
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.384$^{***}$ & 3.021$^{***}$ & -1.637$^{***}$ & 15.252$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.080$^{*}$ & 0.024$^{}$ & 0.056$^{***}$ & -0.024$^{}$ \\
& (0.041) & (0.044) & (0.014) & (0.044) \\
 \textsf{LogReturns} & -0.036$^{***}$ & -0.010$^{*}$ & -0.026$^{***}$ & 0.010$^{*}$ \\
& (0.010) & (0.006) & (0.008) & (0.006) \\
 \textsf{Volatility} & 0.372$^{***}$ & 0.046$^{}$ & 0.326$^{***}$ & -0.046$^{}$ \\
& (0.081) & (0.066) & (0.049) & (0.066) \\
 $\log\textsf{FeeRevenue}$ &  -0.997$^{***}$ & -0.163$^{*}$ & -0.834$^{***}$ & 0.163$^{*}$ \\
& (0.103) & (0.095) & (0.057) & (0.095) \\
 \textsf{Markout} & -0.063$^{***}$ & -0.088$^{***}$ & 0.025$^{***}$ & 0.088$^{***}$ \\
& (0.012) & (0.009) & (0.009) & (0.009) \\
\midrule
 Observations & 37104 & 37104 & 37104 & 37104 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.341 & 0.031 & 0.537 & 0.031 \\
\bottomrule 
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} 
\end{tabular}%
}
\label{table:baseline}
\end{table}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (All Aggregators)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.384$^{***}$ & 3.021$^{***}$ & -1.637$^{***}$ & 15.252$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.083$^{**}$ & 0.030$^{}$ & 0.053$^{***}$ & -0.030$^{}$ \\
& (0.038) & (0.040) & (0.015) & (0.040) \\
 \textsf{LogReturns} & -0.036$^{***}$ & -0.011$^{*}$ & -0.026$^{***}$ & 0.011$^{*}$ \\
& (0.011) & (0.006) & (0.008) & (0.006) \\
 \textsf{Volatility} & 0.357$^{***}$ & 0.040$^{}$ & 0.317$^{***}$ & -0.040$^{}$ \\
& (0.076) & (0.064) & (0.049) & (0.064) \\
 $\log\textsf{FeeRevenue}$ &  -0.928$^{***}$ & -0.125$^{}$ & -0.804$^{***}$ & 0.125$^{}$ \\
& (0.108) & (0.097) & (0.055) & (0.097) \\
 \textsf{Markout} & -0.061$^{***}$ & -0.087$^{***}$ & 0.026$^{***}$ & 0.087$^{***}$ \\
& (0.011) & (0.009) & (0.009) & (0.009) \\
 \textsf{Competition} & 0.224$^{***}$ & 0.111$^{}$ & 0.113$^{***}$ & -0.111$^{}$ \\
& (0.062) & (0.070) & (0.030) & (0.070) \\
 \textsf{Internalization} & 0.167$^{***}$ & 0.136$^{***}$ & 0.031$^{}$ & -0.136$^{***}$ \\
& (0.050) & (0.032) & (0.026) & (0.032) \\
\midrule
 Observations & 37104 & 37104 & 37104 & 37104 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.366 & 0.055 & 0.546 & 0.055 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (UniswapX Only)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
const & 1.384$^{***}$ & 3.021$^{***}$ & -1.637$^{***}$ & 15.252$^{***}$ \\
& (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.069$^{*}$ & 0.019$^{}$ & 0.050$^{***}$ & -0.019$^{}$ \\
& (0.039) & (0.042) & (0.014) & (0.042) \\
 \textsf{LogReturns} & -0.034$^{***}$ & -0.009$^{}$ & -0.025$^{***}$ & 0.009$^{}$ \\
& (0.011) & (0.006) & (0.008) & (0.006) \\
 \textsf{Volatility} & 0.354$^{***}$ & 0.037$^{}$ & 0.317$^{***}$ & -0.037$^{}$ \\
& (0.079) & (0.065) & (0.050) & (0.065) \\
 $\log\textsf{FeeRevenue}$ &  -0.939$^{***}$ & -0.132$^{}$ & -0.807$^{***}$ & 0.132$^{}$ \\
& (0.110) & (0.097) & (0.056) & (0.097) \\
 \textsf{Markout} & -0.061$^{***}$ & -0.087$^{***}$ & 0.026$^{***}$ & 0.087$^{***}$ \\
& (0.012) & (0.009) & (0.009) & (0.009) \\
 \textsf{Competition} & 0.219$^{***}$ & 0.108$^{}$ & 0.110$^{***}$ & -0.108$^{}$ \\
& (0.064) & (0.071) & (0.030) & (0.071) \\
 \textsf{Internalization} & 0.053$^{***}$ & 0.054$^{***}$ & -0.000$^{}$ & -0.054$^{***}$ \\
& (0.021) & (0.020) & (0.007) & (0.020) \\
\midrule
 Observations & 37104 & 37104 & 37104 & 37104 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.356 & 0.042 & 0.545 & 0.042 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\paragraph{WETH--Stable Pairs Only} \text{}

\begin{table}[H] \centering
\caption{
Baseline Regression Model (\ref{equation1}) with Decomposition (\ref{equation2}) $+$ (\ref{equation3})
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.586$^{***}$ & 3.114$^{***}$ & -1.528$^{***}$ & 15.165$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.117$^{**}$ & 0.067$^{}$ & 0.050$^{***}$ & -0.067$^{}$ \\
& (0.052) & (0.059) & (0.017) & (0.059) \\
 \textsf{LogReturns} & -0.169$^{}$ & -0.210$^{*}$ & 0.042$^{}$ & 0.210$^{*}$ \\
& (0.151) & (0.109) & (0.177) & (0.109) \\
 \textsf{Volatility} & 0.342$^{***}$ & 0.096$^{}$ & 0.246$^{***}$ & -0.096$^{}$ \\
& (0.107) & (0.106) & (0.049) & (0.106) \\
 $\log\textsf{FeeRevenue}$ &  -1.109$^{***}$ & -0.276$^{**}$ & -0.833$^{***}$ & 0.276$^{**}$ \\
& (0.136) & (0.130) & (0.055) & (0.130) \\
 \textsf{Markout} & -0.111$^{***}$ & -0.195$^{***}$ & 0.084$^{***}$ & 0.195$^{***}$ \\
& (0.029) & (0.030) & (0.006) & (0.030) \\
\midrule
 Observations & 22863 & 22863 & 22863 & 22863 \\
 N. of groups & 22 & 22 & 22 & 22 \\
 $R^2$ & 0.386 & 0.084 & 0.606 & 0.084 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} 
\end{tabular}%
}
\label{table:baseline}
\end{table}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (All Aggregators)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.586$^{***}$ & 3.114$^{***}$ & -1.528$^{***}$ & 15.165$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.121$^{***}$ & 0.078$^{}$ & 0.043$^{**}$ & -0.078$^{}$ \\
& (0.043) & (0.051) & (0.017) & (0.051) \\
 \textsf{LogReturns} & -0.149$^{}$ & -0.188$^{*}$ & 0.039$^{}$ & 0.188$^{*}$ \\
& (0.159) & (0.111) & (0.177) & (0.111) \\
 \textsf{Volatility} & 0.307$^{***}$ & 0.071$^{}$ & 0.236$^{***}$ & -0.071$^{}$ \\
& (0.095) & (0.098) & (0.042) & (0.098) \\
 $\log\textsf{FeeRevenue}$ &  -1.047$^{***}$ & -0.247$^{**}$ & -0.800$^{***}$ & 0.247$^{**}$ \\
& (0.129) & (0.124) & (0.050) & (0.124) \\
 \textsf{Markout} & -0.111$^{***}$ & -0.195$^{***}$ & 0.084$^{***}$ & 0.195$^{***}$ \\
& (0.029) & (0.030) & (0.006) & (0.030) \\
 \textsf{Competition} & 0.184$^{***}$ & 0.072$^{}$ & 0.112$^{***}$ & -0.072$^{}$ \\
& (0.061) & (0.070) & (0.026) & (0.070) \\
 \textsf{Internalization} & 0.172$^{**}$ & 0.159$^{***}$ & 0.013$^{}$ & -0.159$^{***}$ \\
& (0.070) & (0.049) & (0.030) & (0.049) \\
\midrule
 Observations & 22863 & 22863 & 22863 & 22863 \\
 N. of groups & 22 & 22 & 22 & 22 \\
 $R^2$ & 0.408 & 0.107 & 0.615 & 0.107 \\
\bottomrule 
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (UniswapX Only)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.587$^{***}$ & 3.119$^{***}$ & -1.532$^{***}$ & 15.160$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.098$^{**}$ & 0.053$^{}$ & 0.045$^{**}$ & -0.053$^{}$ \\
& (0.047) & (0.057) & (0.018) & (0.057) \\
 \textsf{LogReturns} & -0.097$^{}$ & -0.079$^{}$ & -0.018$^{}$ & 0.079$^{}$ \\
& (0.160) & (0.074) & (0.160) & (0.074) \\
 \textsf{Volatility} & 0.334$^{***}$ & 0.101$^{}$ & 0.232$^{***}$ & -0.101$^{}$ \\
& (0.105) & (0.119) & (0.051) & (0.119) \\
 $\log\textsf{FeeRevenue}$ &  -1.019$^{***}$ & -0.174$^{}$ & -0.845$^{***}$ & 0.174$^{}$ \\
& (0.137) & (0.148) & (0.064) & (0.148) \\
 \textsf{Markout} & -0.075$^{***}$ & -0.109$^{***}$ & 0.035$^{***}$ & 0.109$^{***}$ \\
& (0.011) & (0.014) & (0.006) & (0.014) \\
 \textsf{Competition} & 0.180$^{***}$ & 0.069$^{}$ & 0.111$^{***}$ & -0.069$^{}$ \\
& (0.066) & (0.076) & (0.025) & (0.076) \\
 \textsf{Internalization} & 0.029$^{}$ & 0.044$^{}$ & -0.015$^{*}$ & -0.044$^{}$ \\
& (0.027) & (0.028) & (0.008) & (0.028) \\
\midrule
 Observations & 22875 & 22875 & 22875 & 22875 \\
 N. of groups & 22 & 22 & 22 & 22 \\
 $R^2$ & 0.385 & 0.045 & 0.614 & 0.045 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\clearpage
\paragraph{L2 Application Pools Only} \text{}

\begin{table}[H] \centering
\caption{
Baseline Regression Model (\ref{equation1}) with Decomposition (\ref{equation2}) $+$ (\ref{equation3})
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 2.412$^{***}$ & 4.359$^{***}$ & -1.947$^{***}$ & 13.896$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.122$^{*}$ & 0.042$^{}$ & 0.080$^{***}$ & -0.042$^{}$ \\
& (0.067) & (0.070) & (0.021) & (0.070) \\
 \textsf{LogReturns} & -0.038$^{***}$ & -0.002$^{}$ & -0.035$^{***}$ & 0.002$^{}$ \\
& (0.011) & (0.008) & (0.009) & (0.008) \\
 \textsf{Volatility} & 0.269$^{***}$ & -0.002$^{}$ & 0.272$^{***}$ & 0.002$^{}$ \\
& (0.087) & (0.071) & (0.053) & (0.071) \\
 $\log\textsf{FeeRevenue}$ &  -1.004$^{***}$ & -0.172$^{*}$ & -0.831$^{***}$ & 0.172$^{*}$ \\
& (0.119) & (0.090) & (0.063) & (0.090) \\
 \textsf{Markout} & -0.083$^{***}$ & -0.161$^{***}$ & 0.078$^{***}$ & 0.161$^{***}$ \\
& (0.026) & (0.020) & (0.020) & (0.020) \\
\midrule
 Observations & 25286 & 25286 & 25286 & 25286 \\
 N. of groups & 26 & 26 & 26 & 26 \\
 $R^2$ & 0.337 & 0.049 & 0.563 & 0.049 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} 
\end{tabular}%
}
\label{table:baseline}
\end{table}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (All Aggregators)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 2.412$^{***}$ & 4.359$^{***}$ & -1.947$^{***}$ & 13.896$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.120$^{**}$ & 0.047$^{}$ & 0.073$^{***}$ & -0.047$^{}$ \\
& (0.058) & (0.061) & (0.021) & (0.061) \\
 \textsf{LogReturns} & -0.040$^{***}$ & -0.004$^{}$ & -0.036$^{***}$ & 0.004$^{}$ \\
& (0.011) & (0.008) & (0.009) & (0.008) \\
 \textsf{Volatility} & 0.267$^{***}$ & 0.001$^{}$ & 0.266$^{***}$ & -0.001$^{}$ \\
& (0.078) & (0.065) & (0.054) & (0.065) \\
 $\log\textsf{FeeRevenue}$ &  -0.931$^{***}$ & -0.126$^{}$ & -0.805$^{***}$ & 0.126$^{}$ \\
& (0.124) & (0.096) & (0.063) & (0.096) \\
 \textsf{Markout} & -0.084$^{***}$ & -0.161$^{***}$ & 0.077$^{***}$ & 0.161$^{***}$ \\
& (0.024) & (0.020) & (0.019) & (0.020) \\
 \textsf{Competition} & 0.260$^{***}$ & 0.158$^{*}$ & 0.102$^{***}$ & -0.158$^{*}$ \\
& (0.074) & (0.082) & (0.032) & (0.082) \\
 \textsf{Internalization} & 0.197$^{***}$ & 0.179$^{***}$ & 0.019$^{}$ & -0.179$^{***}$ \\
& (0.067) & (0.045) & (0.031) & (0.045) \\
\midrule
 Observations & 25286 & 25286 & 25286 & 25286 \\
 N. of groups & 26 & 26 & 26 & 26 \\
 $R^2$ & 0.371 & 0.090 & 0.570 & 0.090 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\clearpage
\subsection{Longer Prediction Horizon}

\paragraph{3 Days}  \text{}

\begin{table}[H] \centering
\caption{
Baseline Regression Model (\ref{equation1}) with Decomposition (\ref{equation2}) $+$ (\ref{equation3})
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.377$^{***}$ & 3.008$^{***}$ & -1.631$^{***}$ & 15.264$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.088$^{**}$ & 0.032$^{}$ & 0.057$^{***}$ & -0.032$^{}$ \\
& (0.043) & (0.043) & (0.015) & (0.043) \\
 \textsf{LogReturns} & -0.039$^{**}$ & -0.021$^{*}$ & -0.018$^{}$ & 0.021$^{*}$ \\
& (0.017) & (0.011) & (0.013) & (0.011) \\
 \textsf{Volatility} & 0.309$^{***}$ & 0.035$^{}$ & 0.274$^{***}$ & -0.035$^{}$ \\
& (0.082) & (0.063) & (0.051) & (0.063) \\
 $\log\textsf{FeeRevenue}$ &  -0.959$^{***}$ & -0.231$^{***}$ & -0.728$^{***}$ & 0.231$^{***}$ \\
& (0.100) & (0.079) & (0.049) & (0.079) \\
 \textsf{Markout} & -0.087$^{***}$ & -0.156$^{***}$ & 0.069$^{**}$ & 0.156$^{***}$ \\
& (0.020) & (0.028) & (0.030) & (0.028) \\
\midrule
 Observations & 36996 & 36996 & 36996 & 36996 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.310 & 0.068 & 0.452 & 0.068 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} 
\end{tabular}%
}
\label{table:baseline}
\end{table}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (All Aggregators)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
const & 1.377$^{***}$ & 3.008$^{***}$ & -1.631$^{***}$ & 15.264$^{***}$ \\
& (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.091$^{**}$ & 0.037$^{}$ & 0.053$^{***}$ & -0.037$^{}$ \\
& (0.039) & (0.039) & (0.015) & (0.039) \\
 \textsf{LogReturns} & -0.039$^{**}$ & -0.021$^{**}$ & -0.018$^{}$ & 0.021$^{**}$ \\
& (0.017) & (0.011) & (0.013) & (0.011) \\
 \textsf{Volatility} & 0.294$^{***}$ & 0.029$^{}$ & 0.265$^{***}$ & -0.029$^{}$ \\
& (0.077) & (0.061) & (0.051) & (0.061) \\
 $\log\textsf{FeeRevenue}$ &  -0.896$^{***}$ & -0.195$^{**}$ & -0.701$^{***}$ & 0.195$^{**}$ \\
& (0.104) & (0.082) & (0.049) & (0.082) \\
 \textsf{Markout} & -0.090$^{***}$ & -0.157$^{***}$ & 0.067$^{**}$ & 0.157$^{***}$ \\
& (0.020) & (0.030) & (0.029) & (0.030) \\
 \textsf{Competition} & 0.212$^{***}$ & 0.109$^{}$ & 0.103$^{***}$ & -0.109$^{}$ \\
& (0.061) & (0.066) & (0.030) & (0.066) \\
 \textsf{Internalization} & 0.157$^{***}$ & 0.131$^{***}$ & 0.026$^{}$ & -0.131$^{***}$ \\
& (0.050) & (0.033) & (0.026) & (0.033) \\
\midrule
 Observations & 36996 & 36996 & 36996 & 36996 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.332 & 0.091 & 0.459 & 0.091 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (UniswapX Only)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.377$^{***}$ & 3.008$^{***}$ & -1.631$^{***}$ & 15.264$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.077$^{*}$ & 0.026$^{}$ & 0.051$^{***}$ & -0.026$^{}$ \\
& (0.041) & (0.041) & (0.014) & (0.041) \\
 \textsf{LogReturns} & -0.037$^{**}$ & -0.020$^{*}$ & -0.017$^{}$ & 0.020$^{*}$ \\
& (0.017) & (0.011) & (0.013) & (0.011) \\
 \textsf{Volatility} & 0.291$^{***}$ & 0.026$^{}$ & 0.265$^{***}$ & -0.026$^{}$ \\
& (0.081) & (0.062) & (0.052) & (0.062) \\
 $\log\textsf{FeeRevenue}$ &  -0.905$^{***}$ & -0.202$^{**}$ & -0.704$^{***}$ & 0.202$^{**}$ \\
& (0.106) & (0.083) & (0.050) & (0.083) \\
 \textsf{Markout} & -0.089$^{***}$ & -0.156$^{***}$ & 0.067$^{**}$ & 0.156$^{***}$ \\
& (0.020) & (0.029) & (0.029) & (0.029) \\
 \textsf{Competition} & 0.207$^{***}$ & 0.106$^{}$ & 0.101$^{***}$ & -0.106$^{}$ \\
& (0.062) & (0.067) & (0.029) & (0.067) \\
 \textsf{Internalization} & 0.051$^{**}$ & 0.048$^{**}$ & 0.003$^{}$ & -0.048$^{**}$ \\
& (0.020) & (0.019) & (0.007) & (0.019) \\
\midrule
 Observations & 36996 & 36996 & 36996 & 36996 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.323 & 0.078 & 0.458 & 0.078 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\paragraph{7 Days} \text{}

\begin{table}[H] \centering
\caption{
Baseline Regression Model (\ref{equation1}) with Decomposition (\ref{equation2}) $+$ (\ref{equation3})
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.366$^{***}$ & 2.994$^{***}$ & -1.628$^{***}$ & 15.275$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.097$^{**}$ & 0.037$^{}$ & 0.060$^{***}$ & -0.037$^{}$ \\
& (0.044) & (0.044) & (0.015) & (0.044) \\
 \textsf{LogReturns} & -0.025$^{}$ & -0.023$^{}$ & -0.002$^{}$ & 0.023$^{}$ \\
& (0.021) & (0.017) & (0.013) & (0.017) \\
 \textsf{Volatility} & 0.248$^{***}$ & 0.023$^{}$ & 0.224$^{***}$ & -0.023$^{}$ \\
& (0.079) & (0.060) & (0.048) & (0.060) \\
 $\log\textsf{FeeRevenue}$ &  -0.890$^{***}$ & -0.241$^{***}$ & -0.650$^{***}$ & 0.241$^{***}$ \\
& (0.103) & (0.078) & (0.051) & (0.078) \\
 \textsf{Markout} & -0.086$^{***}$ & -0.148$^{***}$ & 0.063$^{}$ & 0.148$^{***}$ \\
& (0.023) & (0.036) & (0.043) & (0.036) \\
\midrule
 Observations & 36827 & 36827 & 36827 & 36827 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.271 & 0.069 & 0.362 & 0.069 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} 
\end{tabular}%
}
\label{table:baseline}
\end{table}


\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (All Aggregators)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.366$^{***}$ & 2.994$^{***}$ & -1.628$^{***}$ & 15.275$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.100$^{**}$ & 0.043$^{}$ & 0.056$^{***}$ & -0.043$^{}$ \\
& (0.040) & (0.040) & (0.015) & (0.040) \\
 \textsf{LogReturns} & -0.027$^{}$ & -0.025$^{}$ & -0.002$^{}$ & 0.025$^{}$ \\
& (0.021) & (0.017) & (0.013) & (0.017) \\
 \textsf{Volatility} & 0.234$^{***}$ & 0.018$^{}$ & 0.216$^{***}$ & -0.018$^{}$ \\
& (0.075) & (0.058) & (0.049) & (0.058) \\
 $\log\textsf{FeeRevenue}$ &  -0.834$^{***}$ & -0.208$^{***}$ & -0.625$^{***}$ & 0.208$^{***}$ \\
& (0.107) & (0.081) & (0.051) & (0.081) \\
 \textsf{Markout} & -0.088$^{***}$ & -0.149$^{***}$ & 0.061$^{}$ & 0.149$^{***}$ \\
& (0.022) & (0.038) & (0.042) & (0.038) \\
 \textsf{Competition} & 0.192$^{***}$ & 0.095$^{}$ & 0.096$^{***}$ & -0.095$^{}$ \\
& (0.063) & (0.067) & (0.032) & (0.067) \\
 \textsf{Internalization} & 0.144$^{***}$ & 0.126$^{***}$ & 0.018$^{}$ & -0.126$^{***}$ \\
& (0.049) & (0.034) & (0.025) & (0.034) \\
\midrule
 Observations & 36827 & 36827 & 36827 & 36827 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.290 & 0.089 & 0.368 & 0.089 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

\begin{table}[H] \centering
\caption{
Model (\ref{equation4}) with External Liquidity Variables (UniswapX Only)
}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm} 
>{\centering\arraybackslash}p{2.3cm}}
\toprule
& (1) & (2) & (3) & (4) \\
& $\log\textsf{\,v3Spread}$ & $\log\textsf{\,CFv2Spread}$ & $\log\textsf{\,v3S/CFv2S}$ & $\log\textsf{\,TVL}$ \\
\midrule
% const & 1.366$^{***}$ & 2.994$^{***}$ & -1.628$^{***}$ & 15.275$^{***}$ \\
% & (0.000) & (0.000) & (0.000) & (0.000) \\
 $\log\textsf{GasPrice}$ &  0.087$^{**}$ & 0.032$^{}$ & 0.055$^{***}$ & -0.032$^{}$ \\
& (0.041) & (0.042) & (0.015) & (0.042) \\
 \textsf{LogReturns} & -0.025$^{}$ & -0.023$^{}$ & -0.002$^{}$ & 0.023$^{}$ \\
& (0.021) & (0.017) & (0.013) & (0.017) \\
 \textsf{Volatility} & 0.232$^{***}$ & 0.016$^{}$ & 0.216$^{***}$ & -0.016$^{}$ \\
& (0.078) & (0.059) & (0.049) & (0.059) \\
 $\log\textsf{FeeRevenue}$ &  -0.842$^{***}$ & -0.215$^{***}$ & -0.626$^{***}$ & 0.215$^{***}$ \\
& (0.109) & (0.081) & (0.052) & (0.081) \\
 \textsf{Markout} & -0.087$^{***}$ & -0.149$^{***}$ & 0.061$^{}$ & 0.149$^{***}$ \\
& (0.022) & (0.037) & (0.042) & (0.037) \\
 \textsf{Competition} & 0.188$^{***}$ & 0.092$^{}$ & 0.096$^{***}$ & -0.092$^{}$ \\
& (0.064) & (0.067) & (0.032) & (0.067) \\
 \textsf{Internalization} & 0.050$^{**}$ & 0.045$^{**}$ & 0.004$^{}$ & -0.045$^{**}$ \\
& (0.020) & (0.019) & (0.008) & (0.019) \\
\midrule
 Observations & 36827 & 36827 & 36827 & 36827 \\
 N. of groups & 36 & 36 & 36 & 36 \\
 $R^2$ & 0.283 & 0.077 & 0.368 & 0.077 \\
\bottomrule
\multicolumn{5}{l}{Pool and day fixed effects are included; standard errors are clustered at the pool level.} \\
\textit{Note:} & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}%
}
\label{table:baseline}
\end{table}

==> sections/outline.tex <==
\section{outline, do not include in the end}

\paragraph{timeline}
\begin{itemize}
    \item \textcolor{red}{EoW of Sep 22th, wrap up analysis}
    \item \textcolor{red}{Sep 26th, input introduction, regression results, definitions. Send for comments by EoD}
    \item EoW of Sep 29th, first draft ready to circulate a little bit
    \item Week of Sep 30 - Oct 6, collect feedback and work on robustness checks
    \item Monday, wrap up edits
    \item Tuesday, wrap up edits
    \item Wednesday Submission DDL: AoE 8th October 2024 (potentially AoE 11th)
\end{itemize}


\paragraph{\textcolor{blue}{What we can say}}
\begin{itemize}
    \item we identify some factors on date t that drives (forecasts) liquidity on date t+1, consistent with theory and findings in previous work
    \item by introducing a \textit{v2 counterfactual spread} metric, we can (i) evaluate how much concentration of liquidity in a v3 pool is and (ii) identify the channel through which this happens (i.e. either through more capital deployed, or through higher concentration)
    \item we use quasi-experimental approaches to find the effect of market events on liquidity
    \begin{itemize}
        \item protocol deployments on new chains has a temporary but not permanent effect on liquidity in existing chains
        \item introducing new sources of liquidity, e.g UniswapX, has an effect on liquidity that increases in UniswapX volume
    \end{itemize}
\end{itemize}

\paragraph{Some additional questions}
\begin{itemize}
    \item does v2 counterfactual spread in v3 pools behave similarly to actual v2 spread
    \item how does capital deployed / concentration on t affect themselves on t+1
    \item does source of UniswapX liquidity matter (filler inventory vs on-chain routing)
\end{itemize}

\paragraph{\textcolor{blue}{Sample}}
\begin{itemize}
    \item Period: may 2021 to july 31 2024
    \item Chain / Pools: ETH, Polygon, OP, ARB; WETH-USDC, WETH-USDT, WETH-WBTC; 5bp and 30bp pools; v3 only (but maybe v2 as well)
\end{itemize}

\paragraph{\textcolor{blue}{Depenedent Variables}}

\begin{itemize}
    \item spread
    \item v2 counterfactual spread
    \item difference between v3 and v2 spread
    \item total value locked
\end{itemize}

\paragraph{\textcolor{blue}{Indepenedent Variables}}

\begin{itemize}
    \item Chain level: Average gas price
    \item Pair level: Token price returns, token price volatility
    \item Pool level: Fee revenue, markout (both are normalized by tvl)
    \item $\mathbbm{1}\{\text{First week of deployment on next chain}\}$, $\mathbbm{1}\{\text{Deployed on next chain}\}$
    \item Uniswap X Volume (separate by liquidity source?)
\end{itemize}

\paragraph{Robustness checks}

\begin{itemize}
    \item longer lags
    \item different start days from deployment
    \item different length for deploy days
\end{itemize}


\paragraph{\textcolor{blue}{results / plots to show}}
\begin{itemize}
    \item \textcolor{red}{exploratory data analysis: plots of spread, v2-v3 spread}
    \item \textcolor{blue}{panel data results}
\end{itemize}

\paragraph{\textcolor{blue}{Literature Review}}
\begin{itemize}
    \item Liquidity Misallocation on Decentralized Exchanges \footnote{\url{https://papers.ssrn.com/sol3/papers.cfm?abstract_id=4281293}}
    \item Fragmentation and Optimal Liquidity Supply on Decentralized Exchanges \footnote{\url{https://papers.ssrn.com/sol3/papers.cfm?abstract_id=4267429}}
    \item Implied Impermanent Loss: A Cross-Sectional Analysis of Decentralized Liquidity Pools \footnote{\url{https://papers.ssrn.com/sol3/papers.cfm?abstract_id=4811111}}
    \item How to measure the liquidity of cryptocurrency markets?\footnote{\url{https://www.sciencedirect.com/science/article/pii/S0378426620303022}}
\end{itemize}
